DPU-v2: Energy-efficient execution of irregular directed acyclic graphs

A growing number of applications like probabilistic machine learning, sparse linear algebra, robotic navigation, etc., exhibit irregular data flow computation that can be modeled with directed acyclic graphs (DAGs). The irregularity arises from the seemingly random connections of nodes, which makes the DAG structure unsuitable for vectorization on CPU or GPU. Moreover, the nodes usually represent a small number of arithmetic operations that cannot amortize the overhead of launching tasks/kernels for each node, further posing challenges for parallel execution. To enable energy-efficient execution, this work proposes DAG processing unit (DPU) version 2, a specialized processor architecture optimized for irregular DAGs with static connectivity. It consists of a tree-structured datapath for efficient data reuse, a customized banked register file, and interconnects tuned to support irregular register accesses. DPU-v2 is utilized effectively through a targeted compiler that systematically maps operations to the datapath, minimizes register bank conflicts, and avoids pipeline hazards. Finally, a design space exploration identifies the optimal architecture configuration that minimizes the energy-delay product. This hardware-software co-optimization approach results in a speedup of 1.4$\times$, 3.5$\times$, and 14$\times$ over a state-of-the-art DAG processor ASIP, a CPU, and a GPU, respectively, while also achieving a lower energy-delay product. In this way, this work takes an important step toward enabling an embedded execution of emerging DAG workloads.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> rebuttal.tex <==

\onecolumn
\section*{Summary of modifications addressing reviewer's questions}
The key concerns/questions from reviewers are highlighted in \textbf{bold} and our response is in \re{blue} fonts.

\subsection*{\textbf{Reviewer \#651A}}
\textbf{(1) "The evaluation includes only two applications, PC and SpTRSV. This gives me the sense that this class of problems (large and irregular but statically known DAGs) is pretty narrow. In conventional sparse computations, irregularity manifests as indirect accesses and data-dependent control flow due to sparsity in data structures. Here, the trick is to unfold all of this computation and encode the irregularity in the code itself (as shown in SpTRSV, where the sparsity pattern of the matrix induces a particular DAG). But in general, that would lead to an unwieldy amount of code. Which brings me to the next point..."}

Response: \re{ Thank you for the query. We would like to emphasize that PC and SpTRSV are not specific applications but rather a \textit{class} of models (PC) or kernels (SpTRSV) that are used in a variety of different applications.
As discussed in \S \ref{sec:introduction}, PC are demonstrated to be useful for several applications like robotic navigation \cite{8967568}, robust image classification \cite{DBLP:conf/icml/StelznerPK19}, human activity recognition \cite{galindez2019towards}, etc. Similarly, SpTRSV is a fundamental linear algebra operation not tied to a single use case, but is rather used in diverse applications like robotic localization and mapping \cite{polok2016accelerated}, wireless communication \cite{wang2016overview}, cryptography \cite{delaplace2018linear}, etc., to name a few.

We believe this class of workloads have sufficiently wide and growing application scope to deserve efforts towards enabling efficient execution, especially for energy-constrained use cases.

The issue of large code size is discussed in the next point.
} \newline

\noindent \textbf{(2) "The key trick here is to unfold computations into large DAGs and compile them. Intuitively, this would blow up the size of the code, but this tradeoff is not evaluated. The design includes 512KB instruction and data memories, and Table 2 shows that the instruction memory consumes most of the dynamic power (26\%), so instruction accesses must be frequent. But what is the actual impact on code size w.r.t. other architectures? Does this limit the size of the problem that can be addressed? Have you compared against adopting a similar approach in a conventional RISC processor, where you unfold all of the computation?"}

Response: \re{ It is indeed correct that unfolding the DAG computation into a list of instructions at compile time leads to an increase in code size compared to the conventional approach of using a \texttt{for} loop iterating over the DAG stored in a compressed sparse row (CSR)-like format and performing indirect memory accesses. However, note that the overall memory footprint (instructions + data) of our approach is in fact LOWER than the CSR datastructure.
For the target workloads, the total memory footprint of instructions and data is 48\% smaller than the size of the CSR datastructure, which is not required in our approach.
This is because the statically generated instructions can encode the edge connectivity information with fewer bits, due to the following reasons.

\begin{itemize}  [itemsep=0em]
    \item For the DAG edges that are mapped to PE-PE connections in the datapath, the pointers/addresses for the source and destination of the edges need not be stored, in contrast to the CSR datastructure which stores the pointers for every edge.
    \item Due to the static mapping of variables to the register file, the address for the source/destination of the edges that are mapped to PE-register or register-PE connections can be specified with a register address (= 11b in our final design configuration) instead of encoding in a global address space of 32/64b like it in the CSR datastructure.
\end{itemize}
This reduction in memory footprint is discussed in \S \ref{sec:mem_footprint} of the revised paper. %\mv{these 2 sentences should stand out more, as they are very important. Maybe move them higher up?}
\newline

\textit{Unfolding computations for conventional processors:} Although not discussed in the paper, we did perform experiments where a DAG is statically unfolded in to a list of operations (instead of a dynamic unfolding with a \texttt{for} loop performing indirect accesses) with an Intel CPU. However, we did not observe any performance gain over the dynamic unfolding.
}
\newline

\noindent \textbf{(3) "The paper does not include a proper comparison against much of the relevant prior work: Table 3 consists of results grabbed from prior papers using different baselines, technology nodes, benchamrks, and system setups. For instance, you have tiny on-chip memories and small problems whereas prior work includes a full-blown memory system. In particular, the SPU [8] shows higher performance than your proposed design, and the power efficiency differences may well stem from targeting a system with high-bandwidth memory rather than on-chip SRAMs. A proper comparison should consist of a controlled experiment where you reimplement or adapt prior techniques in your own framework, running the same workloads."}

Response: \re{ Thank you for raising the concern. We originally targeted relatively small on-chip memories and DAG sizes to compare fairly with DPU \cite{shah2021dpu} that is designed for embedded energy-constrained execution. However, our work is not fundamentally limited to these smaller workloads. To demonstrate the scalability and to fairly compare with SPU \cite{dadu2019towards}, we have now benchmarked our work on the large workloads with up to 3.3M nodes, by synthesizing a larger version of our processor. This is discussed in \S \ref{sec:spu_comparison} of the revised version with resulting speedup and power improvement discussion.
%Furthermore, this work consumes 53$\times$ lower power than SPU for the same workloads. We discuss several architectural differences that could lead to the improved energy efficiency in \S \ref{sec:spu_comparison} of the revised version. 

We hope that the new experiments demonstrate that the proposed architecture can support large DAGs up to 3.3M nodes while still operating at a significantly low power budget, making it highly suitable for the embedded applications.
} \newline

\noindent \textbf{(4) "Though the explanations are generally easy to follow, I initially had a pretty hard time figuring out what the paper actually proposes because the framing is very poor. DAGs are not properly defined, and since the term is widely used in programming languages, I was unclear on what a DAG actually meant until fairly deep in the paper (is each node a set of operations with multiple inputs and outputs? a single operation? is there control flow? is the DAG static or dynamically unfolded?). Many of these questions become clear only after key elements of the paper have been explained (e.g., since the DAG is unfolded/has no control flow, the term irregular accesses is completely different than in the more typical term of irregular applications like sparse linear algebra, where irregularity arises due to indirect data accesses and is not simply a property of the lack of structure of the DAG). The paper would really benefit from using proper definitiions and framing, e.g., a concrete example in sections 1 or 2 (and by concrete, I mean having a small DAG with fleshed-out operations, named nodes, etc., and its equivalent code representation, not just a large graph with red dots that could be anything)."}

Response: \re{Thank you for bringing this to our attention. We have clarified further what a DAG node represents in \S \ref{sec:challenges}. The static unfolding aspect is clarified in \S \ref{sec:compiler}.
} \newline


\subsection*{\textbf{Reviewer \#651B}}
\noindent \textbf{(1) "However, the weakest part of the paper is the evaluation and comparison against prior work and CPU/GPU. There is not much explanation regarding how the proposed architecture outperforms prior work. Was it because the bank conflict is reduced, so the throughput is higher? Or does the design of space exploration help too? The paper will be much stronger if the author can provide a deeper analysis of how the proposed design improves over CPU/GPU and prior DPU[38]."}

Response: \re{ Thank you for pointing out the issue. We have rewritten the state-of-the-art comparison section \S \ref{sec:sota_comparison} in the revised version, with detailed qualitative analysis of \textit{why} this work achieves better performance compared to prior work. Performance results are also added for individual workloads. Furthermore, we have enhanced the comparison with SPU by benchmarking with the same workloads that the SPU work had used and by synthesizing a larger version of our processor. We hope that these improvements and additional experiments enhance the quality of comparison against prior work.} \newline

\noindent \textbf{(2) "The other question for this proposal is how often the static DAG is available at compile time. The DAG for the SpTRSV can be obtained by traversing the input sparse matrix, but some irregular applications, such as BFS, won't have the DAG available at compile time. How would the proposed design handle these irregular applications? Can a runtime dynamically decompose a runtime-generated dependency graph and schedule it onto the special architecture?" and another related questions, "What if an irregular application cannot obtain the static DAG offline?"}

Response: \re{ Thank you for the question. The assumption that the DAG structure is known at compile time is always true for performing inference with PC, similar to performing inference with a deep neural network. This assumption also holds often for SpTRSV, in which either the matrix remain the same and the right-hand side vector changes (which only changes the inputs of the DAG), or the non-zero locations in the matrix remain the same but their numerical values change (which again only changes the inputs of the DAG). In fact, one of the key reasons for the prevalence of using lower-upper (LU) decomposition followed with SpTRSV to solve a system of equations instead of Gaussian elimination is that the sparse matrix often remains the same and the right-hand side vector changes. This allows to perform the decomposition once and only execute SpTRSV for every new RHS vector. Some related discussion is available here\footnote{https://www.sciencedirect.com/topics/mathematics/lu-factorization} and here\footnote{https://www.cl.cam.ac.uk/teaching/1314/NumMethods/supporting/mcmaster-kiruba-ludecomp.pdf}.

We would also like to highlight that the prior works DPU\cite{shah2021dpu}, SPU\cite{dadu2019towards}, CPU multithreading\cite{shah2021graphopt}, and GPU cuSPARSE SpTRSV library\cite{naumov2011parallel} also have an \textit{analysis} phase before the actual execution phase, which analyzes the DAG structure to insert synchronization barriers and/or to partition the DAG for parallel cores. The rationale is similar to ours: the overhead would be amortized by multiple execution of DAGs.

\textbf{\textit{BFS:}} Several works targeting graph BFS like \cite{dadu2021polygraph} also assume that the graph structure is known at compile time as this holds for many applications. This allows them to partition the graph to minimize the communication, fit in the on-chip memory etc. However, in BFS, the execution sequence (even for a static graph) is determined at runtime depending on the source node of the search. Our work does not target such operations, but rather the operations where the execution sequence of nodes can be determined at compile time.
} \newline

\noindent \textbf{(3) "Why in figure 1 there is GPU performance estimation for PC, but in table 3 there is only SpTRSV?"}

Response: \re{ Fig.~1 reports the GPU performance for PC based on our implementation utilizing layer-wise parallelization, which is inspired from the SpTRSV implementation in Nvidia CuSPARSE library \cite{naumov2011parallel}. As far as we know, there is no efficient open-sourced GPU library/implementation available for PC. In table 3 of the original paper, we only compared the performance with other published prior work. Upon your suggestion, in this revised version, we now also include the comparison with our GPU implementation of PC in \S \ref{sec:sota_comparison} for the sake of completeness.
} \newline

\subsection*{\textbf{Reviewer \#651C}}
\noindent \textbf{(1) "Although preprocessing appears to be improving the performance, it also introduces overhead. Paper needs to analyze the overhead in terms of both execution time and increase in graph size/program size."}

Response: \re{ Thank you for the suggestion. The impact of preprocessing/compilation on the memory footprint is now discussed in \S \ref{sec:mem_footprint}. In summary, the memory footprint (instructions + data) after compilation in fact reduces by 48\% compared to a compressed sparse row(CSR)-like datastructure used to store a DAG. This is because the statically generated instructions can encode the edge connectivity information with fewer bits, due to the following reasons.

\begin{itemize}  [itemsep=0em]
    \item For the DAG edges that are mapped to PE-PE connections in the datapath, the pointers/addresses for the source and destination of the edges need not be stored, in contrast to the CSR datastructure which stores the pointers for every edge.
    \item Due to the static mapping of variables to the register file, the address for the source/destination of the edges that are mapped to PE-register or register-PE connections can be specified with a register address (= 11b in our final design configuration) instead of encoding in a global address space of 32/64b like it in the CSR datastructure.
\end{itemize}

The DAGs remain static across executions, hence the compilation is performed offline and is not impacting the excution performance. this is not clarified in \S \ref{sec:compiler}
%\ns{TODO: Time overhead of compilation. It is not important because the compilation is performed offline as the DAG structure remains static during execution.}
} \newline

\noindent \textbf{(2) "The description of ISA is short. It is not clear how to map the computation to the hardware using these instructions. Additionally, I found the VLIW terminology to be confusing. From the paper, the instructions appear to be CISC instructions."}

Response: \re{Thank you for raising the issue. %\ns{TODO: improve the description of the ISA}.
We say that the instruction set is similar to VLIW to emphasise the use of long instruction words to express parallel operations as opposed to CISC paradigm which can use short instructions to express complex operations. Furthermore, this terminology is inspired from the prior similar works like \cite{ellis1986bulldog}.

We originally used a table with detailed fields of the instructions in the ISA, but that was replaced with fig.~\ref{fig:decoder} due to space constraints.
Unfortunately, due to highly limited space and time constraints we could not manage to include it again.
%\mv{I believe his point is that VLIW implies that 2 or more "traditional instructions" occur at the same cycle. For you it is a bit different, in that instructions just have very long words. This is a matter of taste / definition. Both opinions are understandable. Indeed using similar terminology as other related (relevant) work would be the best argument here.}
%We call it VLIW to keep the similarity with the BUGS compiler paper.
} \newline

\noindent \textbf{(3) "Table 3 only reports the average speedups. However, in order to analyze the benefits of the architecture proposed in the paper, I would like to see more detailed results. I suggest including figures that show speedups for individual applications and graph pairs."}

Response: \re{ Thank you for the suggestion. The results for individual graphs are now reported in \S \ref{sec:sota_comparison} of the revised version. Additionally, a qualitative analysis has also been added to discuss \textit{why} this work could achieves better performance compared to prior work. We hope these improvements would clarify the comparison with prior works and provide useful insights.
} \newline

\noindent \textbf{(4) "Can you utilize the mapping algorithm for graph partitioning on CPUs? If so, it would be beneficial to create a CPU baseline with a similar preprocessing to justify the benefits of the specialized hardware."}

Response: \re{ Thank you for the recommendation. The compilation algorithm is highly tuned for the spatial mapping and the bank allocation for the architecture of this work, and does not have a direct relevance for CPU multithreading. The output of the step 1 (block decomposition) can possibly be mapped to multiple CPU threads, but it requires additional insertion of synchronization barriers, preventing a direct mapping. 

The CPU baseline used in this work \cite{shah2021graphopt} generates acyclic blocks similar to step 1, however the blocks are made highly tailored for CPU execution, and without unnecessarily getting limited by constraint B mentioned in \S \ref{sec:block_decomposition}. Hence, we believe that the baseline used in this work is better suited for CPU than the output of step 1.

Additionally, we would like to highlight that one of the prior specialized processor, DPU \cite{shah2021dpu}, uses the same partitioning algorithm as our CPU baseline and outperforms CPU. Our work outperforms DPU, further strengthening the hypothesis that specialized processor can bring significant benefit over CPU.
%\ns{I don't think I framed it properly. Maybe we should not mention all this extra details. I am moving on in the interest of time and will revisit later.} \mv{I like your reasoning here. You could slightly shorten if you want, but it is convincing.}
} \newline

\noindent \textbf{(5) "In order to argue that the proposed hardware software design can handle arbitrary size DAGs, it would be beneficial to include larger input DAGs. Current workloads are very small. In these cases, systems like GPUs are expected to be underutilized since there is not enough work to utilize the massively parallel system."}

Response: \re{ Thank you for the suggestion. In order to demonstrate the scalability, additional experiments are performed with larger DAGs having upto 3.3M nodes that were used in one of the prior work, SPU \cite{dadu2019towards} by synthesizing a larger version of the processor. The results are reported in \S \ref{sec:spu_comparison} of the revised manuscript. GPU indeed achieves better performance with larger workloads, but still underperforms specialized hardware.
%It can be seen that the GPU still underperforms compared to our work and CPU. 

We hope that these additional experiments show that the proposed hardware/software framework can handle large graphs.
} \newline

\noindent \textbf{(6) "How did you convert the general DAGs into a binary DAG? What is the algorithm used?"}

Response: \re{A custom algorithm is developed that converts a node to imbalanced binary trees. The inputs that are on the critical path of the DAG are made closer to the tree root, such that overall critical path of the DAG is minimized, increasing parallelism. Due to the limited space, the algorithm is not explained in detail but the code will be open sourced for further clarity.
} \newline

\noindent \textbf{(7) "What is the overhead of initial compiler transformations compared to execution time of PC and TRSV? Are the DAGs static in applications or do they change over time? How many iterations of TRSV or PC needed to amortize the cost after the initial compiler transformations?"}

Response: \re{DAGs remains static across executions and the compilation is performed as offline as now clarified in \S \ref{sec:compiler}. Due to the offline nature of compilation, we did not analyzed how many iterations of TRSV and PC are required to amortize the cost.
%\mv{a couple hours sounds bad... It is really a few hours to map 1 DAG to 1 hardware instantiation?}
} \newline

\noindent \textbf{(8) "How do you set the functionality of individual PEs? Are there instructions for setting the functionality?"}

Response: \re{The PE functionality is set with the \texttt{exec} instruction of the ISA \ref{fig:decoder}(a), which contains 2b configuration fields for every PE. 
%The description of ISA is expanded in the revised manuscript (as much as possible under the space constraint) to provide more details \ns{TODO}. We hope that the more elaborate description is now clear.
} \newline

\subsection*{\textbf{Reviewer \#651D}}

\noindent \textbf{(1) "The observation that irregular graphs have a tree-like structure and can be compounded is not a new observation. You really need to do a qualitative and quantitative comparison against works on compound function units.}
\textbf{In fact see Nathan clark's work in the early 2000s: https://cccp.eecs.umich.edu/papers/ntclark-cases06.pdf.}

\textbf{There has been multiple works in compounding operations to mitigate the problem of irregularity.}     

\textbf{https://research.cs.wisc.edu/vertical/papers/2015/isca15-seed.pdf.}

\textbf{Automated Custom Instruction Generation for Domain-Specific Processor Acceleration. IEEE - -Trans. Computers 54(10): 1258-1270 (2005).} 

\textbf{https://courses.cs.washington.edu/courses/cse591n/10wi/Papers/p271-park.pdf.}

\textbf{https://www2.cs.sfu.ca/~ashriram/papers/2016\_MICRO\_CHAINSAW.pdf"}


Response: \re{ Thank you very much for drawing our attention to the related works. In the revised version, these additional works are now discussed in \S \ref{sec:related_works}, as summarized below:

\begin{itemize}
    \item Clark et al. proposed approaches related to this work, in which frequent recurring subgraphs are identified in a DAG \cite{clark2005automated} to determine the most promising datapath structure, and provided an architecture for dynamic mapping of workloads to the datapath at runtime  \cite{clark2004application}. 
%the operations are and integrated transparently with general purpose processors \cite{clark2004application}.
However, \textbf{the number of ports (4 inputs, 2 outputs) of the datapath are severely limited} as a monolithic register file is used, limiting the parallelism of the datapath. This work addresses that by using a banked register file and provides solutions to address conflicts that arise due to banking, allowing a highly parallel datapath with up to 128 read/write ports.
    
    \item Clark et al.'s "Scalable Subgraph Mapping for Acyclic Computation Accelerators" is highly related, enhanced version, of the step 1 of our compiler. Honestly, we missed this work and reinvented a very similar approach, but their experiments show that the speedup over greedy heuristics is 10\% on average. So, the opportunity of performance gain is limited. Furthermore, the rest of the steps in our compiler would still be required in addition to their work.
    
    \item SEED\cite{nowatzki2015exploring} combines an explicit-dataflow architecture with a general purpose processor. \textbf{It focuses on small DAGs within nested loops, which typically contain high proportion of conditional nodes, while this work focuses on large DAGs with no conditional nodes}, requiring a different approach based on high-bandwidth interconnects and banked register file.
    
    \item CGRA Express \cite{park2009cgra} uses a local register file per PE and also has register bypass networks to dynamically fuse operations with the same goal as the PE trees in this work. An advantage of using PE trees is that $X$ PEs can operate with $X+1$ register read ports, while in CGRA Express, $X$ PEs would require $2X$ ports. Furthermore, experiments in \S \ref{sec:interconnect_dse} shows that \textbf{a one-to-one connection of PE and banks would lead to frequent conflicts, revealing that local register files (similar to one-to-one connection) would be insufficient} and a more complex connectivity between the PEs and register banks is essential for good performance
    
    \item Chainsaw \cite{sharifian2016chainsaw} decomposes DAGs into \textit{chains} instead of trees, which is also a promising alternative as multi-input nodes can also be unfolded as chains. The chains are temporally mapped to a PE equipped with a local register file. \textbf{However, the inter-chain communication, which is frequent for irregular DAGs, happens via a central register file accessed with a bus.} This would become a major bottleneck as fig.~\ref{fig:interconnect_dse} shows that a multi-ported register file and high-bandwidth interconnection used in this work are critical for good performance.
\end{itemize}

We hope that the discussion of the related works has improved in the revised manuscript.
} \newline

\noindent \textbf{(2) "Despite 1) I think there are novel aspects e.g., the register banking and operand networks. Here I think again you need to cite and compare against https://groups.csail.mit.edu/cag/raw/documents/hpca\_2003\_scalar\_operand\_networks.pdf"}

Response: \re{Thank you for the suggestion. Our interconnect networks are indeed a type of \textit{scalar operand networks} discussed in the work (which is primarily focused on a 2D mesh operand network). Our networks have different topologies and they are closely coupled with a spatial datapath, significantly complicating the mapping of operations to the datapath and the routing of operands. Furthermore, the conflict-avoiding bank mapping given the network constraints is also novel.
} \newline

\noindent \textbf{(3) "A problem with all prior work is finding enough ILP without memory operations (even if they are regular loops that can be unrolled). It is unclear to me how you fill the pipeline. Does your scheduling assume that all operations in the mapped graph have deterministic latency? What if there is a load operation? Do you split the graph?"}

Respone: \re{In contrast to the normal approach of iterating over a CSR representation of the DAG, we unfold the graphs at compile time and generate DAG-specific instructions. This converts a large proportion of indirect memory loads into register reads. Figure \ref{fig:instr_stat_all_w} show that the compulsory loads for the DAG inputs are minimal compared to other instructions. Thus, ILP without memory instructions is significantly increased.

The loads are limited to the on-chip data memory with a fixed latency, allowing the compiler to statically schedule, predict pipeline hazards, etc. Experiments in \S \ref{sec:spu_comparison} show that DAGs with millions of nodes can fit in a reasonable on-chip memory (2MB).}
\newline
%, majority of the indirect memory accesses get converted to register accesses, avoiding load instructions. \ns{TODO}

\noindent \textbf{(4) "Your whole avoiding destination register fields seem convoluted to me. Correct me if I am wrong. Essentially,}

\textbf{  --- you want VLIW and all instructions to be of the same width}

\textbf{  --- you avoid having to encode the destination register fields by statically scheduling the graphs? could you not statically schedule away the network conflicts as well?
"}

Response: \re{The primary goal of avoiding the destination register is to reduce the length of instructions as much as possible, and reduce the related overheads. We use VLIW terminology in a general sense to indicate that long instruction words are used to express the operations. The length of different instructions are still different after avoiding the destination register fields.

Yes, the optimization is made possible by statically scheduling the graphs. We call a network conflict a bank conflict, in the sense that the input/output port is not able to reach the required bank in that cycle. These conflicts are minimized by the compiler as discussed in \S \ref{sec:pe_bank_allocation}. For the unresolvable conflicts, compiler statically adds a copy instruction (also in \S \ref{sec:pe_bank_allocation}) to shuffle data across banks, and the hardware does not have to dynamically deal with conflicts.
} \newline

\noindent \textbf{(5) "The register conflict avoidance also has a lot of similarities to sparse matrix scratchpads : https://arxiv.org/pdf/2104.12760.pdf . Please cite and compare"}

Response: \re{Thank you for the pointer. Capstan uses an aggressive reordering of request during runtime like the prior work SPU. In contrast, our work avoids the conflicts altogether during the compilation phase, significantly reducing hardware complexity. This work is now discussed in \S \ref{sec:async_vs_sync} of the revised version, along with SPU.} \newline

\subsection*{\textbf{Reviewer \#651E}}

\noindent \textbf{(1) "The tree based systolic array is not new, which can be found in [Kung-1982-Why Systolic Architectures?]."}

Response: \re{Thank you for the comment. We agree that the tree-based datapath has been introduced in the 1980s, and is also recently used in Maeri \cite{kwon2018maeri}. One of our contributions is identifying that 2D systolic arrays are underutilized for the target class of irregular DAGs and that tree-based datapath can reach high utilization. Furthermore, the tree-based datapath in isolation is not sufficient, and the interfacing with banked independent register banks through flexible interconnects is the key to achieving high performance. Furthermore, the mapping of unstructured DAGs to such a datapath while avoiding bank access conflicts is also a highly challenging problem addressed in this work. Thus, the tree-datapath is one of the parts of the whole hardware-software codesign.} 
\newline

\noindent \textbf{(2) "It's also not very convincing about the comparison between 2D- and tree-shaped PE structures (Sec. 2.2). The former supports more subgraphs due to more flexible connections between PEs although requiring more resources, while the latter supports fewer subgraphs because of the limited connections between PEs. For example, the latter only supports binary subgraphs and some PEs will be idle when mapping a subgraph into a tree. The latter is also ineffective for those nodes with big out-degrees, because the multiple direct successors of one node must belong to different subgraphs (in different blocks), which will cause longer lifetime of the intermediate data and other issues. Therefore, could you please give the evidence of figure 3(c) and explain how to keep tree-shaped structures in a high utilization level?"}

Response: \re{Thank you for the question. Indeed, the tree structure is a subset of a 2D array, and all the patterns that can be mapped to the tree, can also be mapped to a 2D array. Our experiment, however, reveals that there are NO patterns in the target DAGs that are significantly larger than the tree and that can be mapped to the 2D array. Hence, the additional PEs in 2D array will remain severely underutilized.

Multiple direct successors of a node is challenging to map even on the 2D array because the other input of the successors will all be different (otherwise they would become a replica of each other) consuming high number of input ports. Again, if there are patterns with such high out-degree nodes in the DAGs that can utilize the 2D array properly, they would have been discovered in our experiment in \S \ref{sec:systolic_vs_tree}.

The experiment is performed with a published datapath scheduler \cite{nowatzki2014scheduling} that uses a discrete optimization solver which provides a guarantee of optimality while identifying the best pattern that can be mapped to the datapath. Hence, it is not possible to utilize the hardware beyond the peak utilization shown in \S \ref{sec:systolic_vs_tree}.

Also, note that we are not claiming that a tree achieves higher throughput than a 2D array, but showing that the hardware usage in 2D array far exceeds the throughput gains. And with increasing number of inputs, the utilization drops severely because the array size increases quadratically, but not improving throughput proportionally.


We hope that the explanation addresses the question.}
\newline

\noindent \textbf{(3) "It is not clear about the cost when performing graph partition in compiling stage."}

Response: \re{ The target DAGs remain static across multiple executions and hence the compilation is supposed to be performed offline, similar to the prior works SPU, DPU, Nvidia cuSPARSE library, etc. discussed in \S \ref{sec:sota_comparison}. The fact that compilation is offline is now clarified in \S \ref{sec:compiler} in the revised manuscript.
} \newline

\noindent \textbf{(4) "The compiler part is not described clearly. Some concepts are not defined. For example, "spatially schedulable", "compatible PEs", and "Compatible banks". It may be better to define the necessary concepts and also describe complex algorithms with pseudo-codes"}

Response: \re{Thank you for bringing this to our attention. In \S \ref{sec:compiler} of the revised manuscripts, these terms are clarified.
% \begin{itemize}
%     \item \textit{Spatially schedulable:} A spatially schedulable subgraph can be fully mapped to the datapath such that each node in the subgraph is mapped to one and only one PE and each edge is mapped to a ... \ns{TODO}.
    
%     \item \textit{Compatible PEs:} A PE is compatible for a node if the topological consistency defined in constraint E can be satisfied for all the nodes in the block after the given node is mapped to the PE.
    
%     \item \textit{Compatible banks:} A bank is compatible to a node, if mapping the node to that bank does not cause a bank conflict with the already mapped nodes.
% \end{itemize}
Due to the space constraint, we could not add detailed pseudocodes to describe the algorithms. To ensure reproducibility and for a further clarity of the algorithms, our codebase for the compiler as well as hardware RTL will be open-sourced.
} \newline

\noindent \textbf{(5) "The workloads are so small that they all fit in the on-chip data memory."}

Response: \re{ We originally benchmarked small workloads as our aim is to enable embedded processing for energy-constrained systems. Furthermore, these workloads were also used in the prior work, DPU \cite{shah2021dpu}, so they allowed fair comparison with it. In the revised version, we have added additional results on larger workloads with upto 3.3M nodes from the SPU work \cite{dadu2019towards} in which the instructions do not fit in the on-chip memory, to demonstrate the scalability of our work.
%Please also note that our approach leads to 48\% lower memory footprint as described in \S \ref{sec:mem_footprint}, which allows the networks that otherwise would have to be stored in external memory to fit in the on-chip memory.
} \newline

\noindent \textbf{(6) "The analysis is somewhat shallow. It's still not much clear why the proposal can achieve better results."}

Response: \re{ Thank you for raising the concern. In \S \ref{sec:sota_comparison} of the revised manuscript, we have added the discussion of the architectural features of this work that contribute to better results compared to prior works. We hope that the improved analysis is able to give useful insights.
} \newline

\noindent \textbf{(7) "While using a 0.3GHz freq at 28nm, energy is more important."}
Response: \re{We agree that depending on the application requirements, energy efficiency can become more important than EDP. We chose EDP as the figure of merit, but if energy is more critical than the min-energy design from fig.~\ref{fig:dse} can be used.} \newline

\noindent \textbf{(8) "How large bandwidth is assumed in this work?"}

Response: \re{The on-chip instruction memory bandwidth is 112.5 GB/s. For the experiments in \S \ref{sec:spu_comparison}, the external memory bandwidth of 256GB/s same as the SPU is used.} \newline

\noindent \textbf{(9) "I am worried about the scalarability. As I understand, the crossbar is costly and the synthesis result is always too optimistic (on the wiring costs). In Table 2 when B=64, the crossbar size is (Bx32-bit)x(Bx32-bit), 2048x2048, which is quite large."}

Response: \re{  Thank you for the question. We took inspiration from DPU\cite{shah2021dpu}, which is a silicon-proven processor, for the feasibility of a 64x64 words crossbar (1 word = 32b) at a target frequency of 300MHz in the 28nm technology. Their post-layout results showed that such a crossbar only consumed 5\% area and 13\% of the entire chip.
We agree that the post-synthesis results may not be fully accurate for such an interconnect, but even if the power of the crossbar is optimistic by 5 folds, our work would still consume significantly lower power than CPU, GPU, SPU, etc.
} \newline

\subsection*{\textbf{Reviewer \#651F}}

\noindent \textbf{(1) "One problem is the lack of performance comparison/scalability results -- Table 3 is really not doing justice to your performance analysis, since all the baselines are using different graphs and different tech etc. A benchmark-by-benchmark comparison with maybe one other baseline accelerator + a strong implementation on CPU or GPU would be very useful."}

Response: \re{ Thank you for the suggestion. For a strong performance comparison, we have added the following results/discussions to \S \ref{sec:sota_comparison} of the revised manuscript.

\begin{itemize}
    \item A benchmark-by-benchmark comparison for our work with DPU, CPU and GPU is added.
    \item To demonstrate scalability and for a fair comparison with SPU, a large version of our processor is synthesized and benchmarked on the large DAGs used in the SPU work.
    \item A detailed qualitative analysis is done to give insights of \textit{why} our work could outperform prior works.
\end{itemize}
We hope that these improvements make the performance analysis fair and insightful. Also, note that the CPU/GPU benchmarking is done using the state-of-the-art implementations/libraries and with the same DAGs that are used for the proposed processor.
} \newline

\noindent \textbf{(2) "The other issue is DPU[38], which is mentioned in passing, but not really discussed in much detail. The GOPS and EDP are in the same range for these designs, so a more detailed analysis seems warranted."}

Response: \re{Thank you for the suggestion. We agree that this work provides modest improvement over DPU because it is also a highly specialized architecture design specifically for DAGs. Section \S \ref{sec:dpu_comparison} is significantly expanded to provide an insight of the architectural differences that lead to the improvements. Fig.~\ref{fig:throughput_all_w} is also added to provide per-workload througput comparison.
} \newline

\noindent \textbf{(3) "Even though I don’t think evaluating SpTRSV is necessary for this paper, it is interesting that it can be implemented as an irregular DAG traversal. Is it expensive to generate the DAG (since it’s presumably dependent on the sparsity pattern), and is that time included in the overall results? Are there other known data-processing applications that can map to dag traversal?"}

Response: \re{ Thank you the question. The DAG for SpTRSV is indeed induced by the sparsity pattern. The compressed sparse row (CSR)-like representation of a sparse matrix can directly be interpreted as a DAG without additional steps. In fact, CSR is also a common format for storing the adjacency matrix that represents the structure of a DAG. So, there is no additional expense to induce a DAG because it is just an alternative interpretation of the sparse matrix datastructures. The compilation process that consumes the DAG and generates the instructions can be slow, but it is assumed to be done offline and the cost is supposed to be amortized across multiple executions of the DAG. Hence, the compilation overhead is not included in the throughput results.

Many linear algebra operations can be represented as DAGs with only computational nodes (and no conditional nodes). For example, a deep neural network with high sparsity can be interpreted as an unstructured DAG. However, the sparsity in real-world DNNs is typically not high enough, leading to some repetitive structures that can be exploited, unlike sparse matrix operations that can be more than 99\% sparse.
} \newline

\noindent \textbf{(4) "Referring to 4.1, why are nearby blocks in DFS order less likely to have dependencies?"}

Response: \re{ The number of dependencies (most of which are false/avoidable as shown in fig.~\ref{fig:compiler_step_1}) increases significantly if a block combines nodes that are far from each other (in terms of the length of the shortest path between them). Hence, we need some measure of "distance" between a pair of nodes while deciding whether to combine them or not in a block. However, computing the shortest path length between every pair of nodes scales at least quadratically with the DAG size, which is too slow for our purpose. 

Hence, we took inspiration from the conventional knowledge in the register allocation literature (see\footnote{Poletto, Massimiliano, and Vivek Sarkar. "Linear scan register allocation." ACM Transactions on Programming Languages and Systems (TOPLAS) 21.5 (1999): 895-913.} for some insights) that a depth-first order is a good heuristic to keep the producer and consumer nodes closer to each other. In other words, the nodes that are closer to each other in a DFS traversal are more likely to have real dependencies between them, and hence would also be "closer" to each other in the DAG. We empirically found that this heuristic worked well for most workloads.
%leads to lower register file size because the variables that are close to each %\ns{TODO}
} \newline

\noindent \textbf{(5) "The algorithms proposed seem topology agnostic. Is there a reason you went with a Tree only? Did you try other things?"}

Response: \re{ The tree structure is a promising candidate because multi-input nodes can be unfolded into a binary tree of operations for spatial mapping to arithmetic operators with 2 inputs. Furthermore, the experiments with the systolic 2D structure (\S \ref{sec:systolic_vs_tree}) revealed that the DAGs do not contain subgraphs that are significantly larger than a tree and that can be mapped to a 2D array. Hence, none of the subset patterns of a 2D array larger than a tree is a promising candidate.

We do not prove that there does not exist any arbitrary pattern (except for the subsets of a 2D array) that is better than a tree. But we also felt that a tree would be a generic pattern that is not overly specialized for some types of DAGs and would have more applicability.
%\mv{Do we really believe it could be? If not, I would leave out this part...} 
%\ns{May be not, but we nowhere prove that this is not possible}.
Hence, we did not further investigated the problem and instead focused our efforts on the challenge of irregular routing of data between the datapath and the register file (which would exist irrespective of the datapath topology), development of a compiler, and a systematic design space exploration.
} \newline

%We briefly investigated this aspect by enumerating the most frequent subgraphs in the target workloads that are smaller than a certain size. The results were typically unbalanced trees with some 
%Although not discussed in the paper, we used 

%As discussed in the point 5 above, we found that different sizes of unbalanced binary trees are frequently repeating in these workloads and different workloads have different size/shape of frequent trees. Hence, we selected the tree structure. Also, note that our experiments with systolic 2D array (\S \sec)


\noindent \textbf{(6) "How scalable is the approach in terms of performance? Is it even conceivable to get to large hardware-trees or \# of banks? Should this be combined with software techniques like partitioning at some point to avoid the super-large crossbars (and use multi-core versions of this instead)?"}

Response: \re{ It would be feasible to increase the number of banks (and hence the size of the crossbar) beyond 64 as the crossbar is not in the critical path yet (the PE multiplier is in the critical path). However, in the design space exploration (\S \ref{sec:efficient_design}), it can be observed that the EDP advantage is limited for increasing $B$ from 32 to 64 and for increasing $D$ from 2 to 3. Hence, we limited our search space to these limits.

If the target workloads have enough parallelism to utilize even more parallel hardware, we think a 128x128 or 256x256 crossbar could be tried. Beyond that, a system with multiple cores each locally having a crossbar, coupled with a software partitioning technique similar to fig. \ref{fig:async_vs_sync}(a) would be a potential candidate for achieving high performance.
} \newline

\noindent \textbf{(7) "This is more of a comment, but it seems like instruction overhead is the major bottleneck. I wonder if you could find repetitive graph structure to avoid having so many instructions?"}

Response: \re{  Thank you for the question. It may appear that the instruction overhead is higher than conventional processors, but the overall memory footprint is in fact 48\% lower compared to a CSR format used to represent the DAG. This is now discussed in \S \ref{sec:mem_footprint} of the revised manuscript. The tree structure can be considered as a repetitive pattern and a very small proportion of instruction bits are needed to program the PE trees. Majority of instructions are spent in configuring the data movement between the PE trees and the register file. Indeed, if a larger repetitive structure can be discovered, the memory footprint of instructions can be further reduced. But overall, generating DAG-specific instructions is still more efficient in terms of memory footprint than using a general datastructure like the CSR.
} \newline


